Follow-the-Perturbed-Leader for Adversarial Markov Decision Processes with Bandit Feedback

We consider regret minimization for Adversarial Markov Decision Processes (AMDPs), where the loss functions are changing over time and adversarially chosen, and the learner only observes the losses for the visited state-action pairs (i.e., bandit feedback). While there has been a surge of studies on this problem using Online-Mirror-Descent (OMD) methods, very little is known about the Follow-the-Perturbed-Leader (FTPL) methods, which are usually computationally more efficient and also easier to implement since it only requires solving an offline planning problem. Motivated by this, we take a closer look at FTPL for learning AMDPs, starting from the standard episodic finite-horizon setting. We find some unique and intriguing difficulties in the analysis and propose a workaround to eventually show that FTPL is also able to achieve near-optimal regret bounds in this case. More importantly, we then find two significant applications: First, the analysis of FTPL turns out to be readily generalizable to delayed bandit feedback with order-optimal regret, while OMD methods exhibit extra difficulties (Jin et al., 2022). Second, using FTPL, we also develop the first no-regret algorithm for learning communicating AMDPs in the infinite-horizon setting with bandit feedback and stochastic transitions. Our algorithm is efficient assuming access to an offline planning oracle, while even for the easier full-information setting, the only existing algorithm (Chandrasekaran and Tewari, 2021) is computationally inefficient.

==> analysis.tex <==
%!TEX root=main.tex
% This file is removed.

In this section, we present a brief analysis of our episodic AMDP algorithm, \Cref{alg:finite-horizon bandit feedback known transition}. 
For our purpose, we introduce the notation of \textit{occupancy measures} \citep{altman1999constrained,neu2012adversarial}. For each policy $\pi\in \Pi$, it induces $H$ occupancy measures $d_\pi^h\in  \triangle(\mathcal S\times \mathcal A)$, $\forall h\in [H]$, where $d_h^{\pi}$ denotes the probability for policy $\pi$ to visit each state-action pair $(s,a)$ at step $h$. Formally, we have
\begin{equation*}
    d_\pi^h(s,a)\triangleq \Pr\left \{s=s^h,a=\pi^h(s^h)\middle \vert s^{h+1}\sim \mathbb P(\cdot\mid s^h,\pi^h(s^h)),s^1\right \}.
\end{equation*}

Then we can rewrite the total regret as
\begin{equation*}
    \mathcal R_K=\E\left [\sum_{k=1}^K \sum_{h=1}^H \langle d_{\pi_k}^h,\ell_k^h\rangle\right ]-\sum_{k=1}^K \sum_{h=1}^H \langle d_{\pi^\ast}^h,\ell_k^h\rangle.
\end{equation*}

Let $p_k(\pi)$ be the probability that our \Cref{alg:finite-horizon bandit feedback known transition} picks $\pi$ at episode $k$. Then the reward collected by our algorithm is then
\begin{equation*}
    \Alg=\E\left [\sum_{k=1}^K \sum_{h=1}^H \langle d_{\pi_k}^h,\ell_k^h\rangle\right ]=\E\left [\sum_{k=1}^K \sum_{\pi\in\Pi}p_k(\pi)\sum_{h=1}^H\langle d_{\pi}^h,\ell_k^h\rangle\right ].
\end{equation*}

Note that the probability distribution $p_k\in \triangle(\Pi)$ is not deterministic, as it will depend on the random choice of previous episodes as well as the randomness in the reward estimator.

\begin{comment}
To bound $\mathcal R_T$, we consider an ``imaginary FTPL'' process where the policy $\pi$ is updated after each \textit{step} $(k,h)\in [K]\times [H]$.
More preciously, we define
\begin{equation*}
    p_k^h(\pi)=\Pr\nolimits_z\left \{\pi=\argmin_{\pi \in \Pi}\left (\sum_{k'=1}^{k-1}\sum_{h'=1}^H\langle d_\pi^{h'},\hat \ell_{k'}^{h'}\rangle+\sum_{h'=1}^{h-1}\langle d_\pi^{h'},\hat \ell_k^{h'}\rangle+\sum_{h'=1}^H\langle d_\pi^{h'},z^{h'}\rangle)\right )\right \}
\end{equation*}

to be the probability of picking policy $\pi$ at step $(k,h)$.\footnote{One may see this definition exactly coincides with the previous one of $p_k^1$, so there is no abuse of notation.} The total ``imaginary loss'' incurred by this imaginary FTPL process is consequently defined by
\begin{equation*}
    \widetilde{\Alg}\triangleq \E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}p_k^h(\pi)\langle d_\pi^h,\ell_k^h\rangle\right ].
\end{equation*}

Consider the ``flattening'' mapping $i\colon [K]\times [H]\to [KH]$ defined by $i(k,h)=(k-1)H+h$. Define $x(i(k,h))=h$ and $\hat \ell(i(k,h))=\hat \ell_k^h$. Then we have
\begin{equation}\label{eq:def of p_k^h}
    p_k^h(\pi)=\Pr\nolimits_z\left \{\pi=\argmin\limits_{\pi\in \Pi}\left (\sum_{i'=1}^{i(k,h)-1}\langle d_\pi^{x(i')},\hat \ell(i')\rangle+\sum_{h='1}^H \langle d_\pi^{h'},z^{h'}\rangle\right )\right \}.
\end{equation}
\end{comment}

This can be viewed as the \textsc{Context-FTPL} algorithm for adversarial contextual bandits proposed by \citet[Algorithm 2]{syrgkanis2016efficient}: For time slot $i(k,h)$, the context is $x(i)=h$ and the loss is $\hat \ell(i)$. A policy $\pi$ under context $h$ will then give linear feature $d_\pi^h$. We add perturbations to each of the contexts, $1,2,\ldots,H$, denoted by $z^1,z^2,\ldots,z^H\in \mathbb R^{SA}$ respectively. At time slot $i(k,h)$, we simply play the best perturbed policy $\pi$.

However, there is a main differences between our setting and theirs: In their setting, the action space (where $\pi(x_t)$ belongs) is binary. However, in our case, $d_\pi^h\in [0,1]^{SA}$ is continuous. This makes their Lemma 10 no longer hold, which is stated as follows:
\begin{lemma}[{\citep[Lemma 10]{syrgkanis2016efficient}}]
For any contexts $x^1,x^2,\ldots,x^T$ and non-negative linear loss functions $\ell^1,\ell^2,\ldots,\ell^T$, suppose that $z^h(s,a)\sim \text{Laplace}(\eta)$, \textsc{Context-FTPL} satisfies
\begin{equation*}
    \E_z\left [\langle \pi^t(x^t),\ell^t\rangle-\langle \pi^{t+1}(x^t),\ell^t\rangle\right ]\le \eta \cdot \E[\langle \pi^t(x^t),\ell^t\rangle^2],\quad \forall 1\le t<T.
\end{equation*}
\end{lemma}

Define $p_k^{H+1}=p_{k+1}^1$ for simplicity.
We first consider the ``imaginary regret'' $\widetilde{\mathcal R_K}\triangleq \widetilde{\Alg}-\Alg^\ast$. By usual FTPL analysis, we can decompose $\widetilde{\mathcal R_K}$ into two terms, Be-the-Perturbed-Leader (BTPL) term and stability term. As $\mathcal R_K=\widetilde{\mathcal R_K}+(\Alg-\widetilde{\Alg})$, we can decompose $\mathcal R_K$ into three terms: BTPL term, stability term and the term $\Alg-\widetilde{\Alg}$ which we called ``imaginary FTPL term''. So we have
\begin{align*}
    \mathcal R_K=\Alg-\Alg^\ast&=\underbrace{\E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}p_k^{h+1}(\pi)\langle d_\pi^h,\ell_k^h\rangle\right ]-\sum_{k=1}^K \sum_{h=1}^H \langle d_{\pi^\ast}^h,\ell_k^h\rangle}_{\text{BTPL term}}\\
    &+\underbrace{\E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}(p_k^{h}(\pi)-p_k^{h+1}(\pi))\langle d_\pi^h,\ell_k^h\rangle\right ]}_{\text{Stability term}}\\
    &+\underbrace{\E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}(p_k^1(\pi)-p_k^h(\pi))\langle d_\pi^h,\ell_k^h\rangle\right ]}_{\text{Imaginary FTPL term}}.
\end{align*}

\subsection{Bounding BTPL Term}
The BTPL term is bounded by the ``be-the-leader lemma'' (see, e.g., \citet[Lemma 7]{syrgkanis2016efficient} and \citet[Lemma 1]{wang2020refined}), whose proof is deferred to the appendix.
\begin{lemma}[Bounding BTPL term]\label{lem:BTPL term for episodic AMDPs}
The BTPL term is bounded by $\frac{H}{\eta}(1+\ln (SA))$, i.e.,
\begin{equation*}
    \E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}p_k^{h+1}(\pi)\langle d_\pi^h,\ell_k^h\rangle\right ]-\sum_{k=1}^K \sum_{h=1}^H \langle d_{\pi^\ast}^h,\ell_k^h\rangle\le \frac H\eta (1+\ln (SA))=\Otil\left (\frac H\eta\right ).
\end{equation*}
\end{lemma}

\subsection{Bounding Stability Term}
Unlike \citet[Lemma 10]{syrgkanis2016efficient}, as our action space is no longer binary \daiyan{How to express this... Seems unnatural to mention adversarial contextual bandits}, we cannot guarantee \daiyan{todo} anymore. Fortunately, we are able to prove the following weakened version:
\begin{lemma}[Single-step Stability]\label{lem:single-step stability}
If $p_k^h$ is calculated via \Cref{eq:def of p_k^h} where $z^h(s,a)$ are independent samples from $\text{Laplace}(\eta)$, $\forall h\in [H],(s,a)\in \mathcal S\times \mathcal A$, we must have
\begin{equation*}
    p_k^{h+1}(\pi)\le p_k^h\exp(\eta \lVert \hat \ell_k^h\rVert_1),\quad p_k^{h+1}(\pi)\ge p_k^h(\pi)\exp(-\eta \lVert \hat \ell_k^h\rVert_1),\quad \forall \pi \in \Pi,(k,h)\in [K]\times [H].
\end{equation*}
\end{lemma}

By summing up \Cref{lem:single-step stability} for all $\pi\in \Pi$ and using the fact that $\exp(-x)\ge (1-x)$, we have
\begin{equation*}
    \sum_{\pi\in \Pi}(p_k^h(\pi)-p_{k}^{h+1}(\pi))\langle d_\pi^h,\hat \ell_k^h\rangle\le \eta \lVert \hat \ell_k^h\rVert_1\cdot  \sum_{\pi \in \Pi} p_k^h(\pi)\langle d_\pi^h,\hat \ell_k^h\rangle,\quad \forall (k,h)\in [K]\times [H].
\end{equation*}

Further notice that $\hat \ell_k^h$ is one-hot (it is yielded via Geometric Re-sampling), so we consequently have
\begin{equation*}
    \sum_{\pi\in \Pi}(p_k^h(\pi)-p_{k}^{h+1}(\pi))\langle d_\pi^h,\hat \ell_k^h\rangle\le \eta \sum_{\pi \in \Pi} p_k^h(\pi)\langle d_\pi^h,(\hat \ell_k^h)^2\rangle,
\end{equation*}

where the square is taken component-wise.
Moreover, applying \Cref{lem:single-step stability} recursively for $h-1$ times gives $p_k^h(\pi)\le p_k^1(\pi)\exp(\eta \sum_{h'=1}^{h-1}\lVert \hat \ell_k^{h'}\rVert_1)$.
By our choice of $\eta$ and $H$, we have $\eta=(HL)^{-1}$. Together with the fact that $\lVert \hat \ell_k^{h'}\rVert=\hat \ell_k^{h'}(s_k^{h'},a_k^{h'})\le L$ (\daiyan{to ref}), the exponent is consequently bounded by $1$.
Henceforth, after taking expectations w.r.t. $\hat \ell_k$ on both sides, we have
\begin{align*}
    &\quad \E\left [\sum_{\pi\in \Pi}(p_k^h(\pi)-p_{k}^{h+1}(\pi))\langle d_\pi^h,\hat \ell_k^h\rangle\right ]
    \le \E\left [\eta \sum_{\pi \in \Pi} p_k^h(\pi)\langle d_\pi^h,(\hat \ell_k^h)^2\rangle\right ]\\
    &\le \E\left [\eta \sum_{\pi \in \Pi} p_k^1(\pi)\exp\left (\eta \sum_{h'=1}^{h-1}\lVert \hat \ell_k^{h'}\rVert_1\right )\langle d_\pi^h,(\hat \ell_k^h)^2\rangle\right ]
    \le e\E\left [\eta \sum_{\pi \in \Pi} p_k^1(\pi)\langle d_\pi^h,(\hat \ell_k^h)^2\rangle\right ]\\
    &=e\eta \sum_{\pi \in \Pi} p_k^1(\pi) \sum_{(s,a)\in \mathcal S\times \mathcal A} d_\pi^h(s,a)\E[(\hat \ell_k^h(s,a))^2\mid \pi].
\end{align*}

By properties of Geometric Re-sampling \daiyan{to ref}, we have
\begin{equation*}
    \E[(\hat \ell_k^h(s,a))^2\mid \pi]\le (\ell_k^h(s,a))^2 (q_k^h(s,a))^{-1}
\end{equation*}

where $q_k^h(s,a)=\sum_{\pi\in \Pi}p_k^1(\pi) d_\pi^h(s,a)$.
Consequently, we have
\begin{align*}
    &\quad \E\left [\sum_{\pi\in \Pi}(p_k^h(\pi)-p_{k}^{h+1}(\pi))\langle d_\pi^h,\hat \ell_k^h\rangle\right ]\\
    &\le e\eta \sum_{(s,a)\in \mathcal S\times \mathcal A} \left (\sum_{\pi\in \Pi}p_k^1(\pi)d_\pi^h(s,a)\right )(\ell_k^h(s,a))^2(q_k^h(s,a))^{-1}
    \\&\le e\eta SA,
\end{align*}

where we used the assumption that $\ell_k^h\in [0,1]^{SA}$. At last, by the fact that $\E[\hat \ell_k^h(s,a)\mid \mathcal F_{k-1}]=(1-(1-q_k^h(s,a))^L)\ell_k^h(s,a)$ (\daiyan{to ref}), we can have the following result.
\begin{lemma}[Bounding Stability Term]\label{lem:stability term for episodic AMDPs}
The stability term is bounded by $e\eta SAHK+\frac{SAHK}{eL}$, i.e.,
\begin{equation*}
    \E\left [\sum_{\pi\in \Pi}(p_k^h(\pi)-p_{k}^{h+1}(\pi))\langle d_\pi^h,\ell_k^h\rangle\right ]\le e\eta SA HK+\frac{SAHK}{eL}.
\end{equation*}
\end{lemma}

\subsection{Bounding Imaginary FTPL Term}
Applying \Cref{lem:single-step stability} recursively for $h-1$ times, we have $p_k^h(\pi)\ge p_k^1(\pi)\exp(-\eta \sum_{h'=1}^{h-1}\lVert \hat \ell_k^{h'}\rVert_1)$ (which is the opposite direction compared to previous section). Using $\exp(-x)\ge 1-x$ again gives
\begin{equation*}
    \sum_{\pi \in \Pi}\sum_{h=1}^H p_k^1(\pi) \langle d_\pi^h,\ell_k^h\rangle\le \sum_{\pi \in \Pi}\sum_{h=1}^H p_k^h(\pi) \langle d_\pi^h,\ell_k^h\rangle+ \sum_{\pi \in \Pi}\sum_{h=1}^H p_k^1(\pi) \langle d_\pi^h,\ell_k^h\rangle \cdot \eta \sum_{h'=1}^{h-1}\lVert \hat \ell_k^{h'}\rVert_1,\quad \forall k\in [K].
\end{equation*}

Now, taking expectation on both sides w.r.t. $\hat \ell_k$ gives
\begin{align*}
    &\quad \E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi} (p_k^1(\pi)-p_k^h(\pi))\langle d_\pi^h,\ell_k^h\rangle\right ]
    \overset{(a)}{\le} \eta HSA \E \left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi}p_k^1(\pi)\langle d_\pi^h,\ell_k^h\rangle\right ]
    \\&\overset{(b)}{\le} \eta H^2SA\cdot \sum_{k=1}^K \sum_{\pi\in \Pi}p_k^1(\pi)
    \overset{(c)}{=}\eta H^2 SAK.
\end{align*}

where (a) used the fact that $\E[\lVert \hat \ell_k^h\rVert_1\mid \mathcal F_{k-1}]\le SA$ (\daiyan{to ref}), (b) used $d_\pi^h\in \triangle(\mathcal S\times \mathcal A)$ and $\ell_k^h\in [0,1]^{SA}$ while (c) used $p_k^1\in \triangle(\Pi)$. To conclude, we have bounded the imaginary FTPL term as following.
\begin{lemma}[Bounding Imaginary FTPL Term]\label{lem:imaginary FTPL term for episodic AMDPs}
The imaginary FTPL term is bounded by
\begin{equation*}
    \E\left [\sum_{k=1}^K \sum_{h=1}^H \sum_{\pi \in \Pi} (p_k^1(\pi)-p_k^h(\pi))\langle d_\pi^h,\ell_k^h\rangle\right ]\le \eta H^2 SAK.
\end{equation*}
\end{lemma}

\subsection{Bounding Regret}
Summing up the results of \Cref{lem:BTPL term for episodic AMDPs,lem:stability term for episodic AMDPs,lem:imaginary FTPL term for episodic AMDPs} and plugging in $\eta=(HL)^{-1}$, $T=HK$ gives
\begin{equation*}
    \mathcal R_K\le \Otil\left (\frac H\eta+\eta SAT+\eta SAHT+\eta SAHT\right ).
\end{equation*}

A optimal choice of $\eta=(\sqrt{SAT})^{-1}$ then gives $\mathcal R_K\le \Otil(H\sqrt{SAT})$, as claimed in \Cref{thm:regret of episodic AMDPs}.

==> finite-horizon-alg.tex <==
%!TEX root=main.tex
% This file is removed.

\subsection{Known Transition Case}
We first give our algorithm for episodic AMDPs with bandit feedback and known transition, as presented in \Cref{alg:finite-horizon bandit feedback known transition}.

The intuition behind \Cref{alg:finite-horizon bandit feedback known transition} is a rather straightforward application of FTPL --- For episode $k\in [K]$, we simply play the policy that minimizes the cumulative perturbed (estimated) loss, i.e.,
\begin{equation*}
    \pi_k=\argmin_{\pi\in \Pi}\left (\sum_{k'=1}^kV^\pi(s^1;\hat \ell_{k'})+V^\pi(s^1;z)\right )=\argmin_{\pi\in\Pi}V^\pi\left (s^1;\sum_{k'=1}^k \hat \ell_{k'}+z\right ).
\end{equation*}

For simplicity, we use $\hat \ell_{1:k}$ to denote the sum $\sum_{k'=1}^k\hat \ell_{k'}$, where the summation is component-wise vector addition.
This algorithm is quite similar to the full-information FTPL algorithm \citep{even2009online}, except for a usage of Geometric Re-sampling procedure \citep{neu2013efficient} to estimate the loss functions. Compared to the usual importance-weighting estimator in OMD-based algorithms (see, e.g., \citet{jin2020learning}),

\begin{algorithm}[thb]
\caption{FTPL for Bandit Feedback and Known Transition Episodic AMDPs}
\label{alg:finite-horizon bandit feedback known transition}
\begin{algorithmic}[1]
\Require{Laplace distribution parameter $\eta$. Geometric Re-sampling parameter $L$.}
\State Sample perturbations $\{z^h\in \mathbb R^{\mathcal S\times \mathcal A}\}_{h\in [H]}$ where $z^h(s,a)\sim \text{Laplace}(\eta)$.
\For{$k=1,2,\ldots,K$}
\State Let $\pi_k=\text{argmax}_{\pi \in \Pi}V^\pi(s^1;\hat \ell_{0:k-1}+z)$.
\For{$h=1,2,\ldots,H$}
\State Observe $s_k^h$ and play $a_k^h=\pi_k(s_k^h)$.
\State Suffer and observe the loss $\ell_k^h(s_k^h,a_k^h)$.
\State Calculate loss estimation $\hat \ell_k^h$ via Geometric Re-sampling \daiyan{TODO}
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

We have the following regret guarantee for \Cref{alg:finite-horizon bandit feedback known transition}, whose proof is sketched in \Cref{sec:sketched analysis} and presented in \Cref{sec:appendix episodic known}.
\begin{theorem}[Regret of \Cref{alg:finite-horizon bandit feedback known transition}]\label{thm:regret of episodic AMDPs known}
For an episodic AMDP with bandit feedback and known transitions, \Cref{alg:finite-horizon bandit feedback known transition} with $\eta=(\sqrt{SAT})^{-1}$ and $L=\sqrt{SAT}/H$ enjoys a regret guarantee of
\begin{equation*}
    \mathcal R_T\le \Otil\left (H\sqrt{SAT}\right ).
\end{equation*}
\end{theorem}

\subsection{Unknown Transition Case}
For the unknown transition case, for each episode, we maintain a confidence set $\mathcal P_k$ of transitions such that $P^\ast\in \mathcal P_k$ with high probability, $\mathcal P_{k+1}\subseteq \mathcal P_k$ and the number of episodes such that $\mathcal P_{k+1}\ne \mathcal P_k$ is at most $\Otil(HSA)$, which is a combination of the transition estimation technique used by \citet{jin2020learning} and \citet{jin2022near}. We also use the upper occupancy measure technique from \citet{jin2020learning} to ensure an under-estimation of losses.

With such choice of confidence sets and losses, we are able to show that the ERROR term is the same as \Cref{alg:finite-horizon bandit feedback known transition} while the STABILITY term will suffer an extra $\Otil(H^2SA)$ additive factor due to the varying confidence sets.
Furthermore, with this type of confidence sets, we are able to use the Extended Value Iteration algorithm \citep{jaksch2010near} to find the ``optimistic'' policy-transition pair $(\pi_k,P_k)$ from $\Pi\times \mathcal P_k$ that minimizes the perturbed losses, which is far more efficient than the optimization process used in OMD-based \citet{jin2020learning} as noticed by \citet{wang2020refined}.

Note that, though the FTPL regret on \textit{estimated} transitions and losses is bounded by $\Otil(H\sqrt{SAT}+H^2SA)$, we will still suffer an $\Otil(HS\sqrt{AT})$ additional regret due to the transition estimation \citep{jin2020learning}. So this algorithm does not break the $\Otil(\text{poly}(H)S\sqrt{AK})$ barrier for episodic AMDPs with unknown transitions.
Due to space limitations, the full algorithm together with the analysis is deferred to \Cref{sec:appendix episodic unknown}, whose regret guarantee is stated in the following algorithm.
\begin{theorem}[Regret of \Cref{alg:appendix finite-horizon bandit feedback unknown transition}]\label{thm:regret of episodic AMDPs unknown}
For an episodic AMDP with bandit feedback and unknown transitions, \Cref{alg:appendix finite-horizon bandit feedback unknown transition} with $\eta=(\sqrt{SAT})^{-1}$ and $L=\sqrt{SAT}$ ensures
\begin{equation*}
    \mathcal R_T\le \Otil \left (HS\sqrt{AT}+H^2SA\right ).
\end{equation*}
\end{theorem}

